Dissections, orientations, and trees, with applications to optimal mesh encoding and to random sampling

We present a bijection between some quadrangular dissections of an hexagon and unrooted binary trees, with interesting consequences for enumeration, mesh compression and graph sampling. Our bijection yields an efficient uniform random sampler for 3-connected planar graphs, which turns out to be determinant for the quadratic complexity of the current best known uniform random sampler for labelled planar graphs [{\bf Fusy, Analysis of Algorithms 2005}]. It also provides an encoding for the set $\mathcal{P}(n)$ of $n$-edge 3-connected planar graphs that matches the entropy bound $\frac1n\log_2|\mathcal{P}(n)|=2+o(1)$ bits per edge (bpe). This solves a theoretical problem recently raised in mesh compression, as these graphs abstract the combinatorial part of meshes with spherical topology. We also achieve the {optimal parametric rate} $\frac1n\log_2|\mathcal{P}(n,i,j)|$ bpe for graphs of $\mathcal{P}(n)$ with $i$ vertices and $j$ faces, matching in particular the optimal rate for triangulations. Our encoding relies on a linear time algorithm to compute an orientation associated to the minimal Schnyder wood of a 3-connected planar map. This algorithm is of independent interest, and it is for instance a key ingredient in a recent straight line drawing algorithm for 3-connected planar graphs [\bf Bonichon et al., Graph Drawing 2005].

==> Texte/bicoloredTrees.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Appendix: Encoding and sampling bicolored planted binary trees}
\setcounter{section}{1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \subfigure[$\mathcal{A}_{\bullet\circ}$,\label{figure:alph_noir_blanc}]{\input{Figures/Alphabet_noir_blanc.pstex_t}}\qquad\qquad
    \subfigure[$\mathcal{A}_{\bullet}$,\label{figure:alph_noir}]{\qquad\includegraphics{Alphabet_noir.eps}\qquad}\qquad
    \subfigure[$\mathcal{A}_{\circ}$.\label{figure:alph_blanc}]{\qquad\includegraphics{Alphabet_blanc.eps}\qquad}
    \caption{The three alphabets for words associated to bicolored
      binary trees.}
    \label{figure:Alphabets}
  \end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Encoding}\label{section:BicoloredTreesCode}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We explain here how to encode a bicolored tree $T\in\mathcal{B}_{ij}'$.
 Doing a depth-first traversal of $T$ from
left to right, we obtain a word $w_{\bullet\circ}$ of length $(2j+1)$
on the alphabet $\mathcal{A}_{\bullet\circ}$ represented on
Figure~\ref{figure:alph_noir_blanc}, see
Figure~\ref{figure:BicoloredTreeToWord} for an example
(the operation of translating to a word being denoted by $\Psi$). It is easy to
see that the sum of the weights of the letters of any strict prefix of
$w_{\bullet\circ}$ is nonnegative and the sum of the weights of the
letters of $w_{\bullet\circ}$ is equal to -1. In addition,
$w_{\bullet\circ}$ is the unique word in its cyclic equivalence-class
that has these two properties.

\begin{figure}
  \begin{center}
    \includegraphics[height=13em]{BicoloredTreeToPairOfWords.eps}
    \caption{A bicolored rooted binary tree, and the corresponding
    words $w_{\bullet\circ}$, $w_{\bullet}$ and $w_{\circ}$.}
    \label{figure:BicoloredTreeToWord}\label{figure:WordToWordPair}
  \end{center}
\end{figure}

Then $w_{\bullet\circ}$ is mapped to a pair
$(w_{\bullet},w_{\circ}):=\Phi(w_{\bullet,\circ})$ of words such that:
\begin{longitem}
\item $w_{\bullet}$ is a word of length $(2j+1)$ on the alphabet
  $\mathcal{A}_{\bullet}$ (represented on
  Figure~\ref{figure:alph_noir}) with $i$ black-node-letters.
\item $w_{\circ}$ is a word of length $2i$ on the alphabet
  $\mathcal{A}_{\circ}$ (represented on
  Figure~\ref{figure:alph_blanc}) with $j$ white-node-letters.
\end{longitem}
Figure~\ref{figure:WordToWordPair} illustrates the
mapping $\Phi$ on an example.

%\begin{figure}
%  \begin{center}
%    \includegraphics[width=5cm]{WordToWordCouple.eps}
%    \caption{The word $w_{\bullet\circ}$ obtained from the binary tree
%      of Figure~\ref{figure:BicoloredTreeToWord} is transformed into a
%      pair of words $(w_{\bullet},w_{\circ})$.}
%    \label{figure:WordToWordPair}
%  \end{center}
%\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Sampling}\label{section:BicoloredTreesSample}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Conversely, let $(w_{\bullet},w_{\circ})$ be a pair of words such that 
$w_{\bullet}$ is of length $(2j+1)$ on
$\mathcal{A}_{\bullet}$ with $i$ black-node-letters and $w_{\circ}$ is
of length $2i$ on $\mathcal{A}_{\circ}$ with $j$ white-node-letters.
First, we associate to this pair a word
$\widetilde{w}_{\bullet\circ}$ of length $(2j+1)$ on
$\mathcal{A}_{\bullet\circ}$ by doing the inverse operation of the
operation $\Phi$, represented on the right of 
Figure~\ref{figure:WordToWordPair}. This
word has the property that the sum of the weights of its letters is
equal to -1.  There is a unique word $w_{\bullet\circ}$ in the
cyclic equivalence-class of $\widetilde{w}_{\bullet\circ}$ such that
 the sum of the weights of the letters of
 any strict prefix is nonnegative. We associate to
$w_{\bullet\circ}$ a binary tree of $\mathcal{B}_{ij}'$ by doing the
inverse of the operation $\Psi$ illustrated 
in Figure~\ref{figure:BicoloredTreeToWord}.

This method allows us to sample objects of $\mathcal{B}_{ij}'$ and
ensures that
\[
|\mathcal{B}_{ij}'|=\frac{1}{2j+1}\binom{2j+1}{i}\binom{2i}{j}.
\]

